Linguistic Fingerprint in Transformer Models: How Language Variation Influences Parameter Selection in Irony Detection

This paper explores the correlation between linguistic diversity, sentiment analysis and transformer model architectures. We aim to investigate how different English variations impact transformer-based models for irony detection. To conduct our study, we used the EPIC corpus to extract five diverse English variation-specific datasets and applied the KEN pruning algorithm on five different architectures. Our results reveal several similarities between optimal subnetworks, which provide insights into the linguistic variations that share strong resemblances and those that exhibit greater dissimilarities. We discovered that optimal subnetworks across models share at least 60% of their parameters, emphasizing the significance of parameter values in capturing and interpreting linguistic variations. This study highlights the inherent structural similarities between models trained on different variants of the same language and also the critical role of parameter values in capturing these nuances.

==> section/Experiments.tex <==
\section{Experiments} \label{sec: Experiments}
This section provides a detailed explanation of the entire process we followed during our experiment. The process began with the variant-specific datasets extraction to the optimal subnetworks search and the transformer architecture tested.

The EPIC corpus contains approximately 3,000 sentences annotated by multiple annotators, resulting in 14,172 records. To create language-variant-specific datasets, we distilled unique sentences from the corpus and applied majority voting based on annotations, with ties resolved by labeling records as "irony." This meticulous process yielded well-balanced datasets, each comprising approximately 600 records.

Five models, each specializing in a single language variant, were trained using the same transformer architecture. After fine-tuning, we used the KEN pruning algorithm to extract the smallest and most efficient subnetwork in each model. This process involves incrementally increasing the number of fine-tuning parameters retained and decreasing those restored to pre-training values, starting from a minimal subset of parameters and expanding it until the pruned model performance matches or exceeds its unpruned counterpart.
Using these optimized subnetworks, we analyzed the internal structures of the models and measured the similarities between the optimized subnetworks across different language variants. 
For each layer, we extracted the corresponding matrices and conducted a meticulous analysis of the positions of the optimal parameters within each optimal subnetwork. This involved an \textit{"in-breadth" analysis}, which identified the parameters present in all optimal models examined and \textit{pairwise comparisons} between models to identify the language variants with the greatest and least similarity, regardless of the model architecture. We conducted these analyses for each architecture under examination on the layers that constitute the attention mechanism or similar structures, as these layers concentrate most of the arithmetic operations of the model and are a strength of the transformer model core structure.

We replicate this experiment across five distinct transformer model architectures, including Bert \cite{devlin2018bert}, DistilBERT \cite{sanh2019distilbert}, DeBERTa \cite{he2020deberta}, Ernie \cite{sun2020ernie} and Electra \cite{clark2020electra}. The provided Fig. \ref{fig:workpath} visually depicts the entire workflow, starting with language variety subset extraction to the resulting optimized subnetworks obtained.

